Visual Sketchpad: Sketching as a Visual Chain of Thought for Multimodal Language Models

Humans draw to facilitate reasoning: we draw auxiliary lines when solving geometry problems; we mark and circle when reasoning on maps; we use sketches to amplify our ideas and relieve our limited-capacity working memory. However, such actions are missing in current multimodal language models (LMs). Current chain-of-thought and tool-use paradigms only use text as intermediate reasoning steps. In this work, we introduce Sketchpad, a framework that gives multimodal LMs a visual sketchpad and tools to draw on the sketchpad. The LM conducts planning and reasoning according to the visual artifacts it has drawn. Different from prior work, which uses text-to-image models to enable LMs to draw, Sketchpad enables LMs to draw with lines, boxes, marks, etc., which is closer to human sketching and better facilitates reasoning. Sketchpad can also use specialist vision models during the sketching process (e.g., draw bounding boxes with object detection models, draw masks with segmentation models), to further enhance visual perception and reasoning. We experiment with a wide range of math tasks (including geometry, functions, graphs, and chess) and complex visual reasoning tasks. Sketchpad substantially improves performance on all tasks over strong base models with no sketching, yielding an average gain of 12.7% on math tasks, and 8.6% on vision tasks. GPT-4o with Sketchpad sets a new state of the art on all tasks, including V*Bench (80.3%), BLINK spatial reasoning (83.9%), and visual correspondence (80.8%). All codes and data are in https://visualsketchpad.github.io/.

==> old/method_v0.tex <==
\section{Visual Sketchpad}
\label{sec:method}

\begin{figure}[t]
    % \left
    \includegraphics[width=1.01\linewidth]{figures/main.png}
    \caption{\weijia{any suggestion on the figrue?} }
    \label{fig:method}
\end{figure}


We introduce \name, a general framework that enables multimodal LMs to draw sketches as intermediate reasoning steps and to use these sketches to facilitate further reasoning. 
We introduce our multimodal interaction framework in \S\ref{sec:method:react}, and explain how we enable LMs to sketch in \S\ref{sec:method:sketch}.
 
\subsection{Multi-turn Interactions with Multimodal Inputs and Outputs}
\label{sec:method:react}
\weijia{should we remove this part or put it into backgroudn + related work }
% Consider a scenario where the multimodal LMs 
We follow the notation of ReAct~\cite{yao2022react}. Given a multimodal query $q$, which is an interleaved sequence of visual and textual inputs, the LM's goal is to solve the task by interacting with the \name environment.
At time step $t$, the model receives an observation $o_t \in \mathcal{O}$ and takes an action $a_t \in \mathcal{A}$ according to some policy $\pi(a_t\mid c_t)$, in which $c_t=(q, o_1, a_1, \cdots, o_{t-1}, a_{t-1}, o_t)$ is the context of the model. 
In prior work, since most LMs only generate text, the observations $o_t$ are text-only, and actions $a_t$ only manipulate text content. In contrast, in our \name framework, \textbf{observations $o_t$ are multimodal, and actions $a_t$ can manipulate both visual and textual contents.} These changes allow LMs to conduct planning and reasoning \nascomment{using?  about?  need a word here} the visual clues it has drawn.
In summary, for each time step $t$, the model conducts the following steps: 

\noindent\textbf{Thought:} Given the current multimodal context $c_t$, the model conduct reasoning over $c_t$, generating text to support future reasoning and acting. For example, for a geometry problem, the LM may decide to draw an auxiliary line between two points on a math diagram. For a multimodal reasoning problem, the LM may decide to draw a box around an object and mark the box with a number. \nascomment{clarify:  does ``deciding'' mean that the LM outputs a description in text of what it will do?  how is the decision different from the next step, action?}

\noindent\textbf{Action:} Based on the thought, the model executes action $a_t$. In \name, this action can manipulate multimodal content. Specifically, the model first writes Python codesthat can realize the plan proposed in the Thought step, and then run the code to generate multimodal content.  We describe this step in detail in \S\ref{sec:method:sketch}.

\noindent\textbf{Observation:} Based on the action $a_t$, the \name environment returns a new observation $o_{t+1}$. The context is updated to $c_{t+1} = (c_t, a_t, o_{t+1})$. The model continues with the thought, action, observation steps for time step $t+1$, reasoning over its prior sketches. \nascomment{what is the observation?  more text?}

The multi-turn interaction terminates at time step $T$ when the model determines that it has gained enough information from the context $c_T$ to answer the query. It will generate a special action \textbf{Terminate} and return the answer. Our \name implementation is based on the AutoGen~\cite{wu2023autogen} framework.


\subsection{Draw on the \name  via Program Generation and Execution}
\label{sec:method:sketch}

\begin{figure*}[htb]
\begin{minipage}[b]{.45\linewidth}
    Prior work that combines LMs with image generation mainly relies on text-to-image generation models to generate images \cite{zhu2022visualize, lu2023multimodal, manas2024improving}. 
    % \nascomment{suggest deleting this, it's not relevant to the argument, which is about shortcomings of text-to-image models: ``However, existing text-to-image models work differently from how humans sketch on whiteboards.''} 
    However, as demonstrated in Figure~\ref{fig:sketch demo}, even the recent ``natively'' multimodal  GPT-4o fails to follow the instructions to generate sketches that are useful for reasoning. To address these challenges, we instead  let LMs sketch by writing Python code in \name. In each \textbf{Action} step, the LM  generates code to sketch and then executes the code. We now discuss the details of action in time step $t$ below.
\end{minipage}
\quad
\begin{minipage}[b]{.5\linewidth}
    \centering
    \vspace{0.05in}
    \includegraphics[width=.7\linewidth]{figures/sketch demo.png}
    \vspace{-0.05in}
    \captionof{figure}{Existing image generation models 
    %\nascomment{propose to cut:  ``work differently from human sketches and''} 
    cannot produce drawings that facilitate complex reasoning. To address this issue, in \name, LMs sketch the diagram using Python code.}
    \label{fig:sketch demo}
\end{minipage}
\end{figure*}

\noindent\textbf{Program generation.} We adopt a similar approach to recent work~\cite{gupta2023visual, surismenon2023vipergpt, hu2023visual}. We prompt the LM with prompts similar to ViperGPT and VPD, which contain a detailed description of available modules in \name to generate multimodal content.  We will introduce the modules in \S\ref{sec:experiments_math} and \S\ref{sec:experiments_vision}. Specifically, there is a special \textit{display} function that allows the LM to ``see'' the image in the next observation $o_{t+1}$. Notice that the prompt does not contain the full implementation of these modules. Instead, it only provides Python function signatures and docstrings. The full prompt is in \S\ref{sec:appendix:prompt}. The LM is expected to generate Python code in a code block, using the provided functions to generate new image and text outputs. 


\noindent\textbf{Modules for sketching.} 
For mathematical tasks, \name uses common Python packages like matplotlib and networkx for plotting. More details are in \S\ref{sec:math-setup}. For vision tasks, the LM can also use \textbf{specialist vision models} during the sketching process. For example, the detection tool draws bounding boxes on the image; the segmentation and mark tool (inspired by SoM~\cite{yang2023setofmark}) draws colorful masks on the image and uses numbers to label segments. We find these specialists possess vital perception skills for visual reasoning tasks, and \name is an effective way to combine them into a multimodal LM. More details are in \S\ref{sec:experiments_vision:tools}. 


\noindent\textbf{Program execution in a Jupyter Notebook environment.}
LMs can sketch for multiple time steps to solve a task. For example, after adding an auxiliary line, the model might find that it needs to add another line. Taking this into consideration, different from prior work~\cite{gupta2023visual, surismenon2023vipergpt, hu2023visual, ma2024mms}, in which all codes are generated and executed once, \name uses a Jupyter Notebook kernel-based program executor. In each time step, the LM has access to all prior codes, variables, and objects. The model just needs to code for the next Notebook block, and we execute the new code block with the same kernel. This design greatly improves \nascomment{relative to what?} the code generation and execution efficiency in \name. 

\noindent\textbf{Debugging based on execution feedback.} 
LMs sometimes generate erroneous code. Inspired by prior work on LM self-debug~\cite{chen2023teaching}, when the code execution has an error, we put the error message in the observation $o_{t+1}$, and the model will refine its code based on this feedback in the next time step.


% \subsection{Multimodal LMs for \name}
% As seen above, a multimodal LM that works well in \name should be good at multi-turn interaction, coding, and multimodal understanding. In all our experiments, we use  GPT-4-turbo-2024-04-09~\cite{gpt4} and GPT-4o-2024-05-13~\cite{gpt4}, since these models possess the above abilities. While we believe open-source LMs will evolve rapidly, we find that existing open-source multimodal LMs do not perform well on multi-turn interaction and coding. Nevertheless, we experiment with a simplified scenario in \S\ref{sec:analysis:open-source}, showing that open-source models using the oracle plan generated by GPT-4o also achieve great performance improvement.

\nascomment{something I don't understand: what training/adaptation/finetuning needs to be done to get the LM to use this stuff?  or is it all in the prompt?  say more about how you make it work, after now have presented what it does ...}

==> old/scratch.tex <==









In the realm of geometry and mathematics, sketching plays a pivotal role in reasoning and problem-solving. It allows individuals to visualize geometric relationships, explore mathematical concepts, and work through complex equations. By drawing shapes, plotting graphs, and sketching diagrams, learners and professionals can better grasp abstract concepts and discover new insights. This hands-on approach to reasoning enhances cognitive processes and fosters a deeper understanding of mathematical principles.

Beyond these specific domains, sketching finds application in various other fields. In design, it is an essential part of the creative process, enabling designers to brainstorm, prototype, and refine ideas. Engineers use sketches to plan and troubleshoot projects, while scientists rely on them to illustrate experimental setups and results. Even in everyday life, sketching helps individuals organize thoughts, plan activities, and solve practical problems.









Sketches can also convey abstract ideas metaphorically, using elements and spatial relations on paper to express abstract elements and relations.  Expressing ideas in a visuo spatial medium makes comprehension and inference easier than in a more abstract medium such as language.  The externality of sketches and similar cognitive tools promotes memory,providing a record that does not rely on unreliable human memory.  They also provide a token for the contents of working memory, relieving the dual burden of holding the content and also simultaneously operating on it.  Instead,computations and inferences can be made on an external representation. (e. g., Kirsch, 1995; Tversky, 2001)  The public nature of sketches allows a community to observe,comment on, and revise the ideas, and enact those revisions in the external representation.Like spoken and written language, sketches are a form of communication.  More than talking, sketches often serve ascommunications for self.  One role of a sketch is to check the completeness and internal consistency of an idea,especially a spatial idea.   A sketch is a literal model of an idea, an existence proof.  Another role of sketches for self is to see new relations and figures.  These newly seen objects and relations can promote new ideas (e. g., Goel,1995; Goldschmidt, 1991, 1994; Shon, 1983; Shon andWiggins, 1992; Suwa, Gero, and Purcell, 2000; Suwa andTversky, 1996, 1997; Suwa, Tversky, Gero, and Purcell,2001). 




Barbara Tversky, a renowned cognitive psychologist, has extensively studied how people use sketches and other spatial representations to think and communicate. Her research underscores that sketching is not merely a method of recording information but a powerful means of understanding and reasoning. According to Tversky, sketching helps externalize thoughts, making abstract concepts more concrete and manipulable. This process of externalization facilitates cognitive tasks by offloading mental computation onto the physical sketch, thereby reducing cognitive load and enhancing problem-solving efficiency.

One of Tversky's key contributions is the idea that sketches serve as a form of "cognitive scaffolding." This concept highlights how sketches support and extend our cognitive capabilities by providing a visual structure that can be manipulated to explore ideas and relationships. In her work, Tversky demonstrates that sketches allow individuals to break down complex problems into more manageable parts, test hypotheses, and discover new patterns and solutions. This iterative process of sketching and re-sketching fosters deeper understanding and creative thinking.

In the realm of geometry and mathematics, Tversky's research shows that sketching aids in visualizing geometric relationships and exploring mathematical concepts. By drawing shapes, plotting graphs, and sketching diagrams, learners can better grasp abstract principles and reason through complex problems. Tversky argues that these visual representations are crucial for spatial reasoning, helping individuals to see connections and relationships that might not be immediately apparent in purely symbolic or numerical form.

